Statistical guarantees for generative models without domination

In this paper, we introduce a convenient framework for studying (adversarial) generative models from a statistical perspective. It consists in modeling the generative device as a smooth transformation of the unit hypercube of a dimension that is much smaller than that of the ambient space and measuring the quality of the generative model by means of an integral probability metric. In the particular case of integral probability metric defined through a smoothness class, we establish a risk bound quantifying the role of various parameters. In particular, it clearly shows the impact of dimension reduction on the error of the generative model.

==> risk_lower_bounds.tex <==
\begin{theorem}\label{thm:risk_lower_bound}
Let $\mathcal P_{n,D}(d,\sigma,\varepsilon)$ be the set of
all distributions of $n$ points $(\bs X_1,\ldots,\bs X_n)$ 
in $\mathbb R^D$ satisfying \hyperlink{AssA}{Assumption A}. If $\mathcal F$ contains the projection onto the first axis $\bs x\in[0,1]^D \mapsto 
x_1\in\mathbb R$, then, denoting by $D_\mathcal{G}$ the diameter of the class $\mathcal{G}$, there exists a universal constant $c_1$ such that
\begin{align}
    \inf_{\hat{g}_n \in \mathcal{G}} \sup_{g^*} \sup_{P^{(n)} \in \mathcal P_{n,D}(d,\sigma,\varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] \geq c_1(\sigma + \varepsilon + e^{-n\varepsilon/3}D_\mathcal{G}).
\end{align}
\end{theorem}

\begin{remark}
\begin{itemize}
    \item The second term is smaller than $\varepsilon/4$ as soon as $n \geq \frac{3}{\varepsilon} \ln(4D_\mathcal{G}/\varepsilon)$. What happens for $n$ small ?
    \item Lower bound on the regret (instead of the risk) is hard to get with this technique.
\end{itemize}
\end{remark}

We split the proof of \Cref{thm:risk_lower_bound} in two propositions, one for the contamination and the other for the noise.

\begin{prop}(Contamination lower bound)
Let $\mathcal P_{n,D}(d,\sigma,\varepsilon)$ be the set of
all distributions of $n$ points $(\bs X_1,\ldots,\bs X_n)$ 
in $\mathbb R^D$ satisfying \hyperlink{AssA}{Assumption A}. If $\mathcal F$ contains the projection onto the first axis $\bs x\in[0,1]^D \mapsto 
x_1\in\mathbb R$, then, denoting by $D_\mathcal{G}$ the diameter of the class $\mathcal{G}$,
\begin{align}
    \inf_{\hat{g}_n \in \mathcal{G}} \sup_{g^*} \sup_{P^{(n)} \in \mathcal P_{n,D}(d,\sigma,\varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] \geq  \varepsilon/2 + e^{-n\varepsilon/3}D_\mathcal{G}.
\end{align}
\end{prop}

\begin{proof}
Since we are only interested in the effect of contamination we set $\sigma=0$ and for clarity we drop dependencies on $\sigma$ in the notations.

\paragraph{Reduction to Huber contamination model.} Note that the set of admissible data distributions $\mathcal{P}_{n, D}(d, \varepsilon)$ comprises the data distributions from Huber's deterministic contamination model \cite[Section 2.2]{bateni2020}, namely data distributions such that a (deterministic) proportion $(1-\varepsilon)$ of the data is distributed according to a reference distribution $P^*$ while the remaining proportion $\varepsilon$ is independently drawn from another distribution $Q$. Therefore, denoting by $\mathcal{P}^{HDC}_{n, D}(d, \varepsilon)$ such distributions, it holds, for any estimator $\hat{g}_n$ and generator $g^*$,
\begin{align}
    \sup_{P^{(n)} \in \mathcal{P}_{n, D}(d, \varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] \geq \sup_{P^{(n)} \in \mathcal{P}^{HDC}_{n, D}(d, \varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)].
\end{align}
Furthermore, let us denote by $\mathcal{P}^{HC}_{n, D}(d, \varepsilon)$ the set of data distributions such that there is a distribution $Q$ defined on the same space as a reference distribution $P^*$ such that the observations $\bs X_1, \dots, \bs X_n$ are independent and drawn from the mixture distribution $(1-\varepsilon)P^* + \varepsilon Q$. Denoting by $D_\mathcal{G}$ the diameter of the class $\mathcal{G}$, \cite[Proposition 1]{bateni2020} states that for any estimator $\hat{g}_n$ and generator $g^*$,
\begin{align}
    \sup_{P^{(n)} \in \mathcal{P}^{HDC}_{n, D}(d, \varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] \geq \sup_{P^{(n)} \in \mathcal{P}^{HC}_{n, D}(d, \varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] - e^{-n\varepsilon/3}D_\mathcal{G}.
\end{align}

\paragraph{Construction of hypothesis.} Let us define the generators $g_1^*, g_2^* : [0, 1]^d \to [0, 1]^D$ as 
\begin{align}
    g_1^*(\bs u) = (1-\varepsilon)u_1 e_1 \text{ and }
    g_2^*(\bs u) = ((1-\varepsilon)u_1 + \varepsilon)e_1, \qquad \text{ for } \bs u=(u_1, \dots, u_d) \in [0, 1]^d.
\end{align}
For contamination distributions $Q_1 \coloneqq (\mathcal{U}([1-\varepsilon, 1]), \delta_0, \dots, \delta_0)$ and $Q_2\coloneqq (\mathcal{U}([0, \varepsilon]), \delta_0, \dots, \delta_0)$ on $[0, 1]^D$, where $\delta_0$ stands for the Dirac measure at $0$, define the contaminated empirical distributions
\begin{align}
    P_1^{(n)} = [(1-\varepsilon) g^*_1\sharp\mu + \varepsilon Q_1]^{\otimes n} \text{ and }
    P_2^{(n)} = [(1-\varepsilon) g^*_2\sharp\mu + \varepsilon Q_2]^{\otimes n}.
\end{align}
One can easily check that $P_1^{(n)}$ and $P_2^{(n)}$ yield the same distribution $P_0^{(n)} \coloneqq [\mathcal{U}([0, 1]), \delta_0, \dots, \delta_0]^{\otimes n}$ which belongs to 
$\mathcal{P}^{HC}_{n, D}(d, \varepsilon)$.
Using the fact that the maximum is greater than the average and the triangular inequality, we obtain
\begin{align}
    \sup_{P^{(n)} \in \mathcal{P}^{HC}_{n, D}(d, \varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] &\geq \frac{1}{2}\inf_{\hat{g}_n \in \mathcal{G}}\left[ \mathbf{E}_{P_1^{(n)}} \mathsf{d}_{\mathcal F} (g_1^*\sharp\mu, \hat{g}_n\sharp\mu) + \mathbf{E}_{P_2^{(n)}} \mathsf{d}_{\mathcal F} (g_2^*\sharp\mu,sup \hat{g}_n\sharp\mu) \right]\\
    &= \frac{1}{2}\inf_{\hat{g}_n \in \mathcal{G}} \mathbf{E}_{P_0^{(n)}}\left[  \mathsf{d}_{\mathcal F} (g_1^*\sharp\mu, \hat{g}_n\sharp\mu) + \mathsf{d}_{\mathcal F} (g_2^*\sharp\mu, \hat{g}_n\sharp\mu) \right]\\
    &\geq \frac{1}{2} \mathsf{d}_{\mathcal F} (g_1^*\sharp\mu, g_2^*\sharp\mu)\\
    &\geq \varepsilon/2.
\end{align}

The last inequality comes from choosing the representer $f(u) = u_1$ to lower bound the supremum in the following inequalities
\begin{align}
    \mathsf{d}_{\mathcal F} (g_1^*\sharp\mu, g_2^*\sharp\mu) &= \frac{1}{1-\varepsilon} \sup_{f \in \mathcal{F}} \bigg\lvert \int_0^{1-\varepsilon} f(u_1, 0, \dots, 0)du_1 - \int_\varepsilon^{1} f(u_1, 0, \dots, 0)du_1 \bigg\rvert\\
    &= \frac{1}{1-\varepsilon} \sup_{f \in \mathcal{F}} \bigg\lvert \int_0^{\varepsilon} f(u_1, 0, \dots, 0)du_1 - \int_{1-\varepsilon}^{1} f(u_1, 0, \dots, 0)du_1 \bigg\rvert\\
    &\geq \frac{1}{1-\varepsilon} \bigg\lvert \int_0^{\varepsilon} u_1du_1 - \int_{1-\varepsilon}^{1} u_1du_1 \bigg\rvert = \varepsilon.
\end{align}
This concludes the proof.
\end{proof}

\begin{prop}(Noise lower bound)
Let $\mathcal P_{n,D}(d,\sigma,\varepsilon)$ be the set of
all distributions of $n$ points $(\bs X_1,\ldots,\bs X_n)$ 
in $\mathbb R^D$ satisfying \hyperlink{AssA}{Assumption A}. If $\mathcal F$ contains the projection onto the first axis $\bs x\in[0,1]^D \mapsto 
x_1\in\mathbb R$, then,
\begin{align}
    \inf_{\hat{g}_n \in \mathcal{G}} \sup_{g^*} \sup_{P^{(n)} \in \mathcal P_{n,D}(d,\sigma,\varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] \geq \sigma/2 .
\end{align}
\end{prop}

\begin{proof}
Let us define the generators $g_1^*, g_2^* : [0, 1]^d \to [0, 1]^D$ as 
\begin{align}
    g_1^*(\bs u) \equiv 0 \text{ and }
    g_2^*(\bs u) \equiv \sigma e_1, \qquad \text{ for } \bs u=(u_1, \dots, u_d) \in [0, 1]^d
\end{align}
and the empirical distributions
\begin{align}
        P_1^{(n)} = [g^*_1\sharp\mu * \delta_{\sigma e_1} ]^{\otimes n} \text{ and }
    P_2^{(n)} = [g^*_2\sharp\mu*\delta_0]^{\otimes n}.
\end{align}
One can easily check that $P_1^{(n)}$ and $P_2^{(n)}$ yield the same distribution $P_0^{(n)} \coloneqq \delta_{\sigma e_1}$ which belongs to 
$\mathcal{P}_{n, D}(d, \sigma, \varepsilon)$. Using the same arguments as for the contamination lower bound it holds
\begin{align}
\inf_{\hat{g}_n \in \mathcal{G}} \sup_{g^*} \sup_{P^{(n)} \in \mathcal P_{n,D}(d,\sigma,\varepsilon)} \mathbf{E}[\mathsf{d}_{\mathcal F} (g^*\sharp\mu, \hat{g}_n\sharp\mu)] &\geq \frac{1}{2}\inf_{\hat{g}_n \in \mathcal{G}} \mathbf{E}_{P_0^{(n)}}\left[  \mathsf{d}_{\mathcal F} (g_1^*\sharp\mu, \hat{g}_n\sharp\mu) + \mathsf{d}_{\mathcal F} (g_2^*\sharp\mu, \hat{g}_n\sharp\mu) \right]\\
&\geq \frac{1}{2} \mathsf{d}_{\mathcal F} (g_1^*\sharp\mu, g_2^*\sharp\mu)\\
    &\geq \sigma/2. 
\end{align}
\end{proof}


% Noise
